Interscript: A dataset for interactive learning of scripts through error feedback

How can an end-user provide feedback if a deployed structured prediction model generates inconsistent output, ignoring the structural complexity of human language? This is an emerging topic with recent progress in synthetic or constrained settings, and the next big leap would require testing and tuning models in real-world settings. We present a new dataset, Interscript, containing user feedback on a deployed model that generates complex everyday tasks. Interscript contains 8,466 data points -- the input is a possibly erroneous script and a user feedback, and the output is a modified script. We posit two use-cases of \ours that might significantly advance the state-of-the-art in interactive learning. The dataset is available at: https://github.com/allenai/interscript.

==> sections/old-notes.tex <==
% from https://docs.google.com/presentation/d/18dHn61Sl0TphWSAjKM4PhW_ymLhFP12bmIkFhpF7nmA/edit#slide=id.g7ad7dbbd70_0_153

2. Oyvind and Pete: Are there examples where a turker complained that their feedback cannot be translated to one edit operation?
> no. This would be the case when the graph is completely wrong-- and model M was never that off. But a good question because hypothetically one could say 

3. Bhavana: Did you find examples where an alternate graph is possible and feedback gets tricky for those cases? or were all possible correct graphs captured by partial order? 
> the original script dataset was from a recent proscript paper https://arxiv.org/abs/2104.08251 . That paper claimed that all possible correct graphs are captured by partial order. in this work, we can use any prior (bad) graph from any model M (we don't train M ourselves but use a previously trained model). Our objective is to make the corrector use the feedback -- and predict edits that this feedback intends



---

Our feedback typically points out to the problem: e.g., you can’t exit a car that is still moving -- not edits that solve this problem!  from NLEdit paper : https://arxiv.org/pdf/2103.14540.pdf

Long Feedback Not Describing an Edit:
you should determine the major record format from the orchestra table and make sure it is arranged in ascending order of number of rows that appear for each major record format.

Long Feedback Describing an Edit: 
replace course id (both) with degree program id, first courses with student enrolment, course description with degree summary name, second courses with degree programs. 

Table 4: Example long feedback that NL-EDIT struggles with. Top: The feedback describes a rewriting of the query rather than how to edit it. Bottom: The initial query has several errors and the feedback enumerates how to edit all of them.



explicit feedback   =  (medium) localizing the node or edge and hoping the model will fix.
                                      (easy) giving an edit and hoping the model will fix the graph.
implicit feedback   = (medium) feedback on why there is an error.
                                     (hard) feedback on a general principle that the error causes to violate.
distractor feedback =  (medium) top-3 feedback from lexically similar topic.
                                      (easy) top-4 feedback from lexically similar topic.

% these use cases cover various kinds of feedbacks that in real world scenarios from terse to detailed and noisy users.

